Spectral estimation of Hawkes processes from count data

This paper presents a parametric estimation method for ill-observed linear stationary Hawkes processes. When the exact locations of points are not observed, but only counts over time intervals of fixed size, methods based on the likelihood are not feasible. We show that spectral estimation based on Whittle's method is adapted to this case and provides consistent and asymptotically normal estimators, provided a mild moment condition on the reproduction function. Simulated datasets and a case-study illustrate the performances of the estimation, notably of the reproduction function even when time intervals are relatively large.

==> answers_to_reviewers.tex <==
# General

Ne pas oublier de mentionner les points suivants :
- Pareto -> Power Law
- Extension au Hawkes non stationnaire (seulement intensité d'immigration)
- Coefficient d'alpha-mélange avec décroissance exponentielle si moment exponentiel sur h*
- Avons remonté le paragraphe sur le non-causal
- Refait simulations + biais / variance décomposition
- Goodness-of-fit test de l'application
- Package sur le CRAN

Acknowledgements : remercier les reviewers.

# Reviewer 1

## Major issues

1. Motivation: Actually the authors give more than an estimation method: they
give a model. Count time-series data is modeled as aggregated point process
data. So why should this model be relevant? Clearly, most count time-series
data are aggregated events. So physically, the data generating process, is an
continuous-time point process. But when the data is already aggregated, why
then not directly fit a (count) time series on this data? If data is provided in an
aggregated way (like daily Corona-deaths), then typically only the aggregated
data is relevant, no? Also in the measles example, a model only has to give
information on daily deaths, and not if there are more deaths in the morning
or in the evening. So I think the authors have to convince the reader why this
approach might be advantageous. I see two lines of argumentation:

The first argument could be, that people for some reason d o (whether it is
clever or not) exactly that: Modeling count time series by point processes.
And they do it in a far less clever way than the submitted paper: they artifi-
cially distribute the counts over the bins so that the data can be treated as a
continuous-time (and simple) point process. So it would be good if the authors
would look our for a couple of examples where Hawkes models are fitted on
aggregated count data and point out that their estimation method is a much
better way.

The second argument could naturally be that the data generation mechanism i
s continuous in time, and that we will also get better models for the aggregated
representation if we try to model the underlying continuous process. I guess
this might be true when the binning is really rough (e.g., counts of quarterly
credit defaults). However, I guess it is not true for the measles example. This
brings me to the next point:

Following your comment, we have strengthened the motivation of the article by describing in more details the approaches commonly taken when faced with aggregated datasets. In particular, we present and illustrate the two natural strategies to estimate Hawkes processes from count data: either by artificially reconstructing the events within the bins as in @Meyer2012, or by adapting a time series estimation method to the case of count data from Hawkes processes, as in @Kirchner2017.
While it is true that our method is not necessary when the bin size is small, recent sanitary events have shown that in epidemiology particularly, data collection is not an easy process, and that aggregating data over weeks rather than days is a natural way to improve the quality of the data.
Therefore, models have to be adapted to this issue.

2. Goodness-of-fit: So we have bin-count data. On this, the authors provide
a method to retrieve Hawkes parameters. Good. But how do we assess the
goodness-of-fit of the calibrated model? The distribution of the bin-counts
under the model is not clear at all, is it? Given the first issue it would be
naturally interesting to find out, whether this model fits the count data better
than, e.g., some kind of discrete-time Poisson autoregression. Now, how could
these two model fits be possibly compared? This goodness-of-fit issue ought
to be discussed in one way or the other.



3. Stationarity issues: The whole theory of the paper relies on stationarity of
the Hawkes process In the simulation study, however, the model simply starts
in 0. Are there no edge effects like that? I think the authors should think
about using some perfect simulation algorithm like in Møller and Rasmussen
(2005) or at least apply some ‘burn in’ time for the study. Then, a problem of
MLE estimation is that we can only calculate the ‘approximate MLE’ (as the
model uses infinite information from the past but the data are finite). I guess,
this is also a problem for Whittle estimation? It would be good if the authors
could say something about this.



4. Pareto decay: The discontinuity discussion of the likelihood in the Pareto-
case on p8 is interesting (I never thought about this!) and distracting (I had
to think about it!) at the same time. Why not work with an alternative
Pareto density (of the form c(a + t) γ−1 , t ≥ 0). Like this the authors would
keep all properties of their arguments, and, in addition they would be able to
perform MLE. What is most irritating is that the shape parameter γ is not
being estimated. Is this true? Why? This is the most interesting parameter!
Maybe the authors want to have the same number of parameters as in the
exponential case? But then, better keep a fixed.



5. Bias: In Figures 2, 5, and 7, we see that for T = 100 the true values are quite
far away from the median of the estimates. I would be interested whether
it is also that far away from the average (some estimate distributions look
quite skew). In other words: I would be interested if the large MSE for large
bin-sizes and short samples is caused more by a high variance or more by a
‘discretization bias’. (As Theorem 3 tells us, this possible ‘discretization bias’
goes to zero (for all ∆) as T goes to infinity.)



6. Multitype case: p12, ‘Nevertheless, we decided to concentrate on the uni-
variate case for brevity and added clarity.’: I agree partly. The usefulness of the
paper would increase if it provided at least notation and formulae for the mul-
titype case in a separate chapter. But I do not no what the AOS-restrictions
on page count do say. Or maybe, as a compromise, the authors could imple-
ment the multitype case, and write something like ‘simulations show that the
method also works in the multitype case’, and provide the code?



7. Code: I spent about one hour to try and make the code run. It looks good
and clear, but I was not able to load it as a package ‘hawkesbow’ from github:
I use

library(devtools)
install_github("fcheysson/hawkesbow")

and obtain

installation of package
‘/var/folders/k0/q1twnhl13kq6jsw9dgs36gxr0000gp/T
//RtmpLOGkNr/file4a175b5eb977/
hawkesbow_0.0.0.9000.tar.gz’ had non-zero exit status

And if I download the files and source them ‘by hand’, then still some ob-
jects/functions are missing. It would be great if this could be fixed in a way
that users can simply download the little package from CRAN and use the
code without further ado. Also some of the questions I had could have been
answered if I had been able to run through the examples.



## Minor minor issues

1. p1: The title is a bit long, isn’t it? Why not only: Spectral estimation of
Hawkes processes from count data (or: from count time series, or: from bin
count sequences). (I do not think that it is very surprising that a Hawkes
process is strongly mixing.) If you look at it from very far away, a Hawkes
process is more or less a homogeneous Poisson process.

We decided to change the title to the one you suggested: 
Spectral estimation of Hawkes processes from count data

2. Use much more equation numbers allover the paper. It would simplify my and
future communications on the paper.

3. Be much more genereous with giving the domain of definition of formulas all
over the paper.

4. Notation: You interpret point processes as measures and not as (random count-
ing) functions nearly throughout. So I would consequently prefer Lebesgue
integrals
$\int_(-\infty,t) f(s)N(\\d s)$ to Stieltje integrals
$\int_{-\infty}^t f(s)\\d N(s)$.

We have modified the integrals accordingly.

5. p2, ‘reproduction kernel’: at this point it is no t clear to the reader that is
meant here. Maybe clarify in sentence with Galton–Watson tree.

We specified that the reproduction function is the intensity of the Poisson offspring process of the Galton--Watson tree.

6. p2, ‘ finance (Bacry, Mastromatteo and Muzy, 2015)’: This is an important
and influential paper. However, Bowsher (2002) and Chavez-Demoulin et al.
(2005) gave finance applications of Hawkes processes long before that.

7. p3: just to be sure I would state at some point that you want the Hawkes
process to be simple. Otherwise, (depending on exact definition of ‘conditional
intensity’) from any simple solution of the Hawkes equation $N$ would yield
infinitely more solutions $N_k (\dd t) \coloneqq kN(\dd t), k \in \mathbb N$.

We clarified that we only consider *simple* locally finite point processes (subsection 2.1).

8. p4: Reconsider spelling of ‘binsize’.

All 'binsize' occurrences are now spelled 'bin size'.

9. p4, DEFINITION: Please provide number. And why not define $X_k$ in terms of
$X_t$ ? Why not give the two processes differnt names? Like: ‘bin-count process’
and ‘bin-count sequence’? Figure not needed.

We changed the definition accordingly.

10. p4, ‘This definition can be adapted to a point process $N$ on$\mathbb R$’. I do not understand why you do not write ‘stationary point process’ here and forget about
‘ts’ resp. ‘ns’ in this definition of the mixing coefficients? For a stationary
point process like the Hawkes process, the set you take the supremum over,
depends of one single number, no? And would this not simplify all calculations
(notations)?

While we first assumed stationarity of the process, the proof of Theorem 1 was written with non-stationary processes in our mind, and it turns out that the alpha-mixing property can be straightforwardly obtained in the case where the immigration intensity $\eta(\cdot)$ is allowed to vary with respect to time.
We thus decided to include this case as a corollary to the Theorem 1 (see Corollary 1).

11. p4: ‘distribution kernel’: before, this is called ‘reproduction kernel’, no? And
why not call it ‘displacement density’? Or ‘displacement distribution’? Actually, this ‘kernel’ has nothing to do with the genealogical structure but only
with the locations of the offspring. So ‘reproduction’ might be misleading.

We have normalised the definitions used throughout the manuscript, and defined and named the terms $\mu$ and $h^\ast$ more clearly in the beginning of the text.
BIRTH TIME DENSITY
ARRIVAL DENSITY

12. p4: in expression $(X_k)_{a\le k<b}$ make clear that $k \in \mathbb Z$. In all filtrations, reconsider open/closed interval boundaries. E.g., as its now, the definition for the
filtrations implies that $X_{−\infty}$ and $X_\infty$ were well defined.

We made clear that $k \in \mathbb Z$ in $\{X_k: k \in \mathbb Z, a \le k \le b\}$, therefore disallowing $k$ from taking the values $-\infty$ or $\infty$.

13. p4, ‘Note that, since $\mathcal F_a^b \subset \mathcal E(a, b]$, we have that $\alpha_X(r) \le \alpha_N(r)$.’: The
conclusion is clear. But the premise? Say, $a = 0$ and $b = 1$. Then, e.g.,
$X_1 = N(1,1 + \Delta]$ is subset of $\mathcal F_a^b$
but not of $\mathcal E(a,b]$.

Thank you for this remark, we have corrected this oversight.

14. p4, Theorem 1: I am not used to the shorthand
$\int h = \ldots$.

We have made the integral clearer.

15. p4: ‘consequence to’ → ‘consequence of’

16. p5: I’m having a hard time deriving definition/property (1) from Daley and
Vere-Jones (2009), Proposition 8.2.I. However, one finds eq.(1) on page 340 in
the same volume – however in a slightly other context. Please elaborate.

We made explicit that using a polarisation argument from equation (8.2.2), we get the desired relation (now equation (2) [TO CHECK] in the manuscript) on the covariance of the counting measure.

17. p6: ‘For the Hawkes process sampled in discrete time on a regular unit time
grid,...’ → (maybe) ‘For the corresponding bin-count sequence, ...’

18. p5/6: Here, we are working with three kinds of spectral representations: The
Bartlett spectrum of a point process, the spectral density of a continuous time
process, and the spectral density of a time series. All these are calculated
similarly but different. It would help the reader, if you gave the definitions.
Maybe inside Proposition 1 and inside Corollary 2?

We specified the definitions of the spectral density functions for both time-continuous and a discrete-time processes, and made explicit how they relate to each other via aliasing.

19. p7, Theorem 2, (A1): Awkward formulation. Better: ‘The true parameter $\theta_0$
belongs to ...’.

20. p7: So, at least asymptotically we have no discretization bias with this method.
Great! However, the variance of the estimates will obviously depend on the
bin-size. Would it be possible to factor out the bin size $\Delta$ from the information
matrices and to (at least heuristically) argue how the diagonal terms of the
covariance matrix of the estimator behave in $\Delta$?

In $\Gamma_\theta$, the derivative of $\mathrm{log} f_\theta(\omega)$ with respect to $\eta$ is simple and does not depend on $\Delta$.
On the other hand, the dependency of $C_{4, \theta}$ on $\Delta$ must be approximately of order $\Delta$, $\propto \Delta^3$ for the fourth-order cumulant spectral density and $\propto \Delta^{-2}$ for the derivative of $1 / f_\theta(\omega)$, ignoring further effects from the term $\widetilde h(\omega / \Delta)$.
This would amount for $\eta$ to a variance that depends approximately linearly on $\Delta$.

However, for $\mu$ and the other parameters that $h^\ast$ may involve, it is not straightforward to factor out the dependency of the partial derivatives on the bin size $\Delta$.
Indeed, even for simple reproduction kernels (exponential and gaussian), we could not derive explicitly the derivative of $log f_\theta(\omega)$, or factor out $\Delta$.

21. p8, eq.: clarify integration boundaries
$\int_{-\infty}^t$, and range of definition (I guess,
$t \in \mathbb R$).

22. Maybe put Figure 2 and 9 in one single figure?



23. In simulation study/data example: Please tell the reader which optimization
routine was used used (including possible choice of starting values and/or
boundary values).

We detailed the optimisation routine (L-BFGS-B), as well as the boundary values given on the parameters.

24. p9: In subsubsection 5.2.1 it is not immediately clear which figure you refer
to.

Added a reference to the figure at the beginning of subsubsection 5.2.1.

25. p9, ‘This can be related to the probabilty that a point has an offspring in the
same bin:’: It think this is not the probability you calculate. The event ‘a
point has an offspring in the same bin’ would have to take into account that
there might be no offspring at all. If I am not mistaken, what you calculate
(and which gives exactly the interpretation you want) is the probability that
‘a point’s parent is in the same bin as the point itself’.

As we formulated, it is not clear whether we consider that there could be no offspring at all. We clarified that it is indeed the probability that both the parent and its offspring belong in the same bin.

26. p10, Figure 3: Nice plot! The dots could be way larger (for my eyes). The
large values for the $\beta$-estimates for $T = 100$ are really very, very large. Was
there maybe a problem with some of the optimization routines? Or might it
have to do with edge-effects? But then, I would expect more problems in the
Pareto-case. Hmm.



27. p10: nice little case study! Eq. at bottom: Again, provide range of definition.
And is this causal??? I guess, no, as ‘infection goes typically forward in time’.
So, as I understand it, this density should be $= 0$ for $t \le \nu$. But then you
would need some factor to make it a probability density. But then: What is
the ‘interquartile range’ on the next page about ... Please clarify.

In the case study, the reproduction kernel of the Hawkes process represents the infectious period of the measles.
Incubation time can be related to the mean parameter $\nu$ of the Gaussian kernel, while the transmission period can be related to the standard error $\sigma$.
However, since the data represents diagnosed cases, it may happen that an offspring is reported before its parent, and therefore we use a non causal Hawkes process to model this situation (one where offsprings can be generated in the past).
In consequence, we moved up the paragraph on non causal Hawkes processes, that we initially had put in the conclusion of the manuscript, just before the case study.
We also clarified the context of the case-study, to better understand why a non causal Hawkes process is needed.

In consequence, the interquartile range here denotes the usual interquartile range for the gaussian distribution, namely the value $1.35 \sigma$.
We note that, with the estimated parameters $\widehat\nu$ and $\widehat\sigma^2$, the estimated probability that there is an offspring before its parent is low, $< 5\%$.

28. p10: ‘We treat the process as stationary because the impact of the seasonality
was small compared to local variability.’: Do I see this from the plot?

The between-week variability was not high enough compared to the within-week variability to justify strong non stationarity (see figure attached).
We decided not to include this figure in the manuscript as it is not decisive nor highly relevant to the novel method we ought to highlight.

[ INCLUDE HERE WEEKLY MONTHPLOT OF DATASET ]

29. A comment on the case study: Regarding the model, I think I would treat
$h^\ast$ as given and fixed or at least use some Bayesian prior for its shape. (I
guess this function is a very well-studied biological property and we know
quite a lot about it.) Then the only parameters left to estimate would be the
immigration rate and the expected reproduction size ‚Äì with much smaller
variance at that.

Indeed, if the transmission function is known in advance or a prior can be set on its shape and / or position, then the other parameters of the model can be estimated with smaller variance.
However, the aim of the case-study was to show that the estimation method developed in the manuscript gives plausible estimates, rather than finding the best estimates for the immigration rate and the expected reproduction size.
Moreover, to our knowledge, there is no consensus on the form of the reproduction function for contagious diseases.

30. I like the very explicit referencing in the proofs-part!

31. p12, Lemma I: At some point one would have to explain to the reader what is
meant by $N(\cdot|y)$. And is this really good notation? N looks like the Hawkes
process itself, no? Ah, OK: You defined this on p.3. But then, maybe refer to
it ...

We now explicitly state in the statement of the Lemma that $N(\cdot | y)$ denotes for the branching process generated by an immigrant at time $y$.

32. p13: ‘...conditioning on ...’

33. p13, better: ‘...of a typical single branching process N(·|0).

34. p13, proof of Lemma 2: If space is short, I would substitute this standard proof
by a reference. And why not put Lemma 2 and Lemma 3 together. Anyway,
the second part of Lemma 2 is just a special case of Lemma 3.

XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXx

35. The whole paper could use much more equation numbers – it would make
communication about the paper much easier.

XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXx

36. p13: Make clear if you start with generation 0 or generation 1! Maybe in
sentence on middle of page: For $k \in \mathbb N_0$, let $Z_k$ be ...

We specified the case $k = 0$.

37. p13: In all formulas here (and the rest of the paper) please specify domain of
definition .



38. p14, Lemma 4(ii): ‘an upper bound’

39. p15, l1: Remove brackets around reference. And reference is not very helpful
as the statement is given there as ‘well-known’. Give proof or provide reference
with proof.

The reference to von Bahr and Esseen has been removed and replaced with a direct proof involving Hölder's inequality.

40. p15, Wright–Fisher process: I have never heard of this process. So either
elaborate, or give reference, or leave away. I think, this backward construction
is quite clear.

As the reference to the Wright-Fisher process was not an insightful remark and the backward construction is clear on its own, we removed the reference.

41. p15, ‘We state a useful Lemma ...’: Awkward. Better: ‘In order to ...we will
need/use the following Lemma:’.

42. p15, Lemma 7: Make explicit that upper bound holds for $s < t, t + r < u, r
>0$.

43. Figure 5: In xlab: Think about if you might prefer hat-notation ($\widehat\eta$ and so on).
Pick ylim a bit larger. Make clear in caption that formula holds for $t \ge a$.

XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXxx


# Reviewer 2

This is a very good paper. In fact, I think this is the best paper I have read in a long time. It seems at first to be about a technical issue, namely strong mixing conditions, but actually is potentially really important as a way of estimating point processes observed using total counts over realistically sized intervals, and the authors suggest estimating them based on a spectral method. 
I only have minor remarks. 

1. On p2 the authors list some applications of Hawkes processes. There are more, some of which are given in the nice review by Reinhart (2018).

Thank you for this review. We have added it as a reference for Hawkes processes and their applications in the introduction of our manuscript.

2. On the bottom of p1 and the 4th line of p2, the authors suggest that clustering and self-exciting are two different things. My understanding is that they are the same. 

Indeed, for Hawkes processes, clustering is a consequence of their properties of self-excitation.
However in general, clustering properties can come from other behaviours, such as heterogeneity, and therefore the two properties are not equivalent.
Furthermore, non-localised self-excitation (for example when the reproduction function decreases very slowly) may not generate observable clustering, as there is an overlap between the offsprings belonging to the different generations.
This is why we decided to talk about both properties, which have been separately invoked to motivate applications in the literature.
%Furthermore, both properties have been separately invoked to justify applications, such as self-excitation for earthquakes, and clustering for contagious diseases.

3. On p3 the authors define the Hawkes process. They should require h to be a density and use the notation K h(t-u) instead of h(t-u), because then the parameter K represents the productivity and is nicely interpretable, and also making h a density can ease the notation in many cases and help with the integral approximation as explained in Schoenberg (2013). 

We followed your recommendation and introduced the decomposition $h = \mu h^\ast$ accordingly.

4. The authors define the background rate eta as constant. In practice, it can be important to let eta vary over space and time, and possibly even depend on covariates. Can the method the authors propose extend to this situation? 

We have extended the alpha-mixing properties for Hawkes processes with time-varying immigration intensity $\eta$ (see Corollary 1).
However, regarding its application, the extension of the Whittle estimation method to non stationary time series requires a precise framework for non stationarity, known as local stationarity @Dahlhaus2012, and new results of asymptotic convergence for its estimator.
To our knowledge, these results do not exist in the literature, and would require a great amount of work; even with a clear strategy, we are not sure we would be able to achieve it.

5. When I try to download hawkesbow from the R depository, I get the error "package ‘hawkesbow’ is not available (for R version 4.0.1)". 

The package is not yet available on the CRAN, but on Github.
It can be installed through the command `devtools::install_github("fcheysson/hawkesbow")`.
We plan to release it on the CRAN as soon as possible, when it is in a more stable state.
XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXxxx

6. On p8, the authors say they cannot compare their method with MLE. Does regular MLE refer to the case where you observe the actual points, and the process is not observed merely over increments? If so, I do not understand why the MLE should be difficult to obtain. 

Regular MLE does indeed refer to the case where we observe the actual points of the process.
With the Pareto kernel, the likelihood has more than $n$ points of discontinuity and those points of discontinuity change with the value of the parameter $a$.
This makes it more difficult to compute the MLE, mainly due to the increase to the complexity of the maximisation algorithm.
However, with a renormalisation of the Pareto kernel, using the power law density instead:
$$h^\ast(t) = \frac{1}{(t+a)^\theta},$$
we have fixed this problem and we now compare the Whittle estimates to the MLE.

7. "seasonality" in misspelled on p11. 

Thank you for the correction.

8. I like how the authors consider the non-causal case on p12, but they are ignoring serious problems and intricacies here. There isn't really such a thing as a non-causal Hawkes process. What the authors mean is a Poisson cluster process, but since the conditional intensity at time t must by definition be predictable and thus only depend on the past, it is simply not correct to write lambda(t) = eta + sum of h(t-u) where the sum is taken over the past and future values of u, and the authors do not state this but it is implicit in their discussion. I think for non-causal point processes, the conditional intensity has to be completely reparameterized differently. 

Indeed, there was an oversight in how we described the non-causal Hawkes process in the manuscript.
Thanks to your remark, we have now made clear that the process should be taken as a Poisson cluster process, and that its conditional intensity function is not tractable (see Subsection 6.1).

Reinhart, A. (2018). A Review of Self-Exciting Spatio-Temporal Point Processes and Their Applications. Statist. Sci. 33(3), 299-318. 

Schoenberg, F.P. (2013). Facilitated estimation of ETAS. Bulletin of the Seismological Society of America, 103(1), 601-605. 

# Reviewer 3

This paper discusses the the strongly mixing condition for univariate, self-exciting, linear
Hawkes processes. The decay rate of the strongly mixing coefficient is derived under a
moment condition on the self-exciting kernel, and is further used to establish limiting results
for a Whittle estimator on the so-called “bin-count” process. The observation on the strongly
mixing condition (Theorem 1) is a neat observation, that might be suitable for a journal on
probability or stochastic processes. However, the current manuscript lacks novelty in its
theoretical results as well as solid statistical motivations. I cannot recommend this paper in
its current state to be published in the Annals of Statistics.

1. This paper considers a very restricted class of point processes: the univariate, self-exciting, linear Hawkes process (Hawkes, 1971). As the authors are aware of, properties of the Hawkes process have been studied extensively (see, among others, Brémaud and Massoulié, 1996; Bacry et al., 2013; Delattre et al., 2016; Chen et al., 2017; Costa et al., 2018) under a variety of conditions, where most of the recent works tackle with dimensionality, inhibition or non-linear link functions. It is well-known that a linear Hawkes process enjoys great analytical tractability. Hence, discussion on this simple, restrictive model is of limited interest from a theoretical prospective.

From a quick read of the proof, it may be straight-forward to generalize the theory to the multivariate case. I would suggest the authors to at least explore how dimensionality affects the strongly mixing condition.

% Dead reviewer, C'est chouette ce qu'on a fait. Le reviewer devrait être heureux. Nous suggérons un couple de petits canards, ou alors un petit Diazépam.

A large part of statistical results and applications make use of the markovian dependence properties of the linear Hawkes process with exponential reproduction function.
Our manuscript is a step forward by providing probabilistic results for the statistical study of a wide class of linear Hawkes processes, with only a mild condition of the moments of the reproduction kernel.
Following your review, we investigated some extensions of the alpha-mixing properties for the linear Hawkes process, but they need further technical developments:

- The multivariate case: One main argument of the proof in the univariate case is that the arrival times $T_i^k$ are independent of the number of offsprings in any given generation $Z_l$, $\forall k, l \in \mathbb N$ and $1 \le i \le Z_k$.
  However, in the multivariate case, this argument does not hold since the distribution function of an inter-arrival time depends on the type of the parent, therefore on the allocation of the types in the preceding generation.
  Further development is needed in order to control the covariance in Lemma \ref{lem:onecluster}.

- Higher dimensionality: Concerning dimensionality, the cluster representation also enables us to define non-causal linear Hawkes processes in $\mathbb R^d$.
  All arguments presented in Appendix \ref{sec:alphamixing} can be generalised to this case, noting that the alpha-mixing coefficient can be defined for point processes in higher dimensions \citep{Poinas2017}.
  Lemma \ref{lem:bigO} must then be adjusted by assuming that there exists $\delta > 0$ such that $\nu_{d + \delta} < \infty$, to ensure integration with respect to the first-moment measure of the centre process.
  This yields alpha-mixing coefficients for the multi-dimensional linear Hawkes process, albeit with a stronger condition on the reproduction kernel.
  However, generalisation of the statistical components of the article is more difficult: while recently the Whittle estimator has been extended to the Gaussian model in any number of dimensions \citep{Guillaumin2020}, there has not yet been any work generalising the results from \citep{Dzhaparidze1986} for alpha-mixing time series to higher dimensions.

- Non-linear Hawkes processes: Finally, following your review we investigated the properties of non-linear Hawkes processes with respect to our problem.
  Let $N$ denote the linear Hawkes process with conditional intensity function
  \begin{equation*}
      \lambda(t) = \eta + \int_{-\infty}^t h(t-u) N(\mathrm d u),
  \end{equation*}
  and $N'$ a non-linear Hawkes process with conditional intensity function 
  \begin{equation*}
      \lambda'(t) = \phi\left( \int_{-\infty}^t h(t-u) N'(\mathrm d u) \right),
  \end{equation*}
  where $\phi$ is a non-negative measurable function.
  We originally thought that properties of strong-mixing of $N'$ could be obtained by comparison of the $\sigma$-algebras of $N$ and $N'$, for example through the Poisson embedding introduced in \citep{Bremaud1996}, then used by \citep{Costa2018} to prove a coupling between the two processes.
  However, this coupling alone does not provide a direct comparison between the two $\sigma$-algebras, since the coupling process depends on the complete past of the non-linear Hawkes process. 

% - Non-linear : perte des bonnes propriétés de dépendance (pas d'équivalence de branchement, donc pas de conservation directe des propriétés de dépendance) (Graham et al. : reconstruction difficile, conditioner proprement ce qui se passe entre les événements difficile ; dans le cas exponentiel, potentiellement possible avec du beta-mixing en s'appuyant sur des propriétés markoviennes)
% - Multivariate : détailler ce qui coince au moment de l'article (indépendance des T_i et des Z_j non valable dans le cas multivarié) et que nous sommes en train de travailler dessus
% - Dimensionalité : travail théorique possible sur des mailles régulières, mais application difficile car maille généralement arbitraire, administrative, et procédés de Fourier inadaptés là-dessus

2. The real-data motivation is ill-founded. In the manuscript, the authors have not shown that the proposed Whittle estimator yields any advantages over existing methods on the bin-counts data. The only case-study the authors provide is on an infectious disease data set (Section 6 of the manuscript). In epidemiology, such data are usually modeled with differential equation systems (e.g., the SEIR model). However, the authors provide no comparisons between their proposal and existing methods. I find it very unconvincing to claim that the proposed approach is appealing (Section 7) given the lack of comparisons — especially so since the model is already very restrictive.

For the kind of datasets that we consider, comparison with the SEIR model i
Estimation of the SEIR model parameters 
Modele SIR = modele de population
Le notre = modele individuel
